Learning Gaussian Policies from Corrective Human Feedback

Learning from human feedback is a viable alternative to control design that does not require modelling or control expertise. Particularly, learning from corrective advice garners advantages over evaluative feedback as it is a more intuitive and scalable format. The current state-of-the-art in this field, COACH, has proven to be a effective approach for confined problems. However, it parameterizes the policy with Radial Basis Function networks, which require meticulous feature space engineering for higher order systems. We introduce Gaussian Process Coach (GPC), where feature space engineering is avoided by employing Gaussian Processes. In addition, we use the available policy uncertainty to 1) inquire feedback samples of maximal utility and 2) to adapt the learning rate to the teacher's learning phase. We demonstrate that the novel algorithm outperforms the current state-of-the-art in final performance, convergence rate and robustness to erroneous feedback in OpenAI Gym continuous control benchmarks, both for simulated and real human teachers.

==> chapters/thingsthataredeleted.tex <==
\subsection{RELATED WORK}

        % This study builds on earlier work that has been conducted within in robotics community, specifically regarding advising and guiding computational agents that learn in a stochastic setting. 
        % not very to the point %JS
        
        Studies that consider learning from feedback in the action domain
        % originally? As of today, we have carlos %JS
        mostly concern the adoption of 'advise'-operators in the learning process \cite[e.g.][]{maclin1996creating,argall2008learning}. The policy was trained by the teacher by suggesting (a sequence of) actions to the agent. These advice-operators however needed to be pre-coded in the algorithm which would hinder general application of the frameworks for non experts. Also, the advice was primarily engaged in a discrete action domain: continuous action domain would require an accurate guess of the action to execute, which was therefore impractical.  
        % Now, continue:
        % A breaktrough was achieved by \citet{celemin2015coach}, who extended corrective feedback to the continuous domain. 
        % A bit on how they did that.
        
        % Uncertainty and confidence measures for policy learning has been researched quite extensively.
        We here discuss two studies with uncertainty/confidence-handling in interactive learning.
        For feedback in the evaluative domain \cite{li2016using} studied the advantages of communicating the state-uncertainty to the teacher in an \ac{AL} framework. 
        % So, ?
        In contrast to the study by
        \cite{knox2009interactively}, where trainers quantified the evaluation of the agent's behavior, \cite{griffith2013policy} motivated that humans have difficulties with the quantification of observed performance. 
        As an alternative, they introduced a framework in which evaluative human feedback was regarded as \textit{policy advise}, and derived a Bayes optimal update rule to convert that into a policy.
        % Uncertainty was used to... (its now not clear how this relates to the scope of the paragraph)
        
        The employment of \ac{AL} in learning processes mostly concerns the inquiry for demonstrations based on uncertainty. For example the study by \cite{grave2013learning}, where the confidence of predictions is used to inquire a suggested sequence of actions from the trainer.
        \ac{AL} is in general applied on settings that inquire extensive human labeling, e.g. \cite{de2008active}, but studies assessing the potential of employing uncertainty in feedback based frameworks is rather conducted limited.
        
        % Dingen als:
        % - Online regression of GP, wanneer worden ze lijpppp
        % - Sparsifications techniques
        % - RL met GP 
        % - Iets met Argall
        % - Active learning
        %     - Active learning for primary drug screening
        %     - Active Learning for High Throughput Screening
        % - Adapting policies nadat ze al gemaakt zijn
        % - DAgger, Active en alles
        % - Advice
        
        % AL is hot topic tegenwoordig. Zie https://www.aaai.org/ocs/index.php
        % /FLAIRS/FLAIRS18/paper/view/17489/16860
        
        % tive Learning with Gaussian Processes for Object Categorization
        % https://ieeexplore.ieee.org/abstract/document/4408844

==> chapters/todo.tex <==
item: GPC-CS veranderen in GPC en GPC-NS in GPC-NS
item: commas around i.e. and e.g.
